Evaluating Correctness and Faithfulness of Instruction-Following Models for Question Answering

Retriever-augmented instruction-following models are attractive alternatives to fine-tuned approaches for information-seeking tasks such as question answering (QA). By simply prepending retrieved documents in its input along with an instruction, these models can be adapted to various information domains and tasks without additional fine-tuning. While the model responses tend to be natural and fluent, the additional verbosity makes traditional QA evaluation metrics such as exact match (EM) and F1 unreliable for accurately quantifying model performance. In this work, we investigate the performance of instruction-following models across three information-seeking QA tasks. We use both automatic and human evaluation to evaluate these models along two dimensions: 1) how well they satisfy the user's information need (correctness), and 2) whether they produce a response based on the provided knowledge (faithfulness). Guided by human evaluation and analysis, we highlight the shortcomings of traditional metrics for both correctness and faithfulness. We then propose simple token-overlap based and model-based metrics that reflect the true performance of these models. Our analysis reveals that instruction-following models are competitive, and sometimes even outperform fine-tuned models for correctness. However, these models struggle to stick to the provided knowledge and often hallucinate in their responses. We hope our work encourages a more holistic evaluation of instruction-following models for QA. Our code and data is available at https://github.com/McGill-NLP/instruct-qa

==> Figures/prompts.tex <==
\begin{figure}[h!]
\small
\begin{tabular}{p{0.96\columnwidth}}
\toprule
\textbf{Instruction 1}\\
\midrule
\texttt{Please answer the following question given the following passages.} \\
\midrule
\textbf{Instruction 2}\\
\midrule
\texttt{Please answer the following question given the following passages. If the answer is not in the passages or cannot be inferred from the passages, respond as ``I don't know''.} \\
\midrule
% \textbf{Instruction 3}\\
% \midrule
% \texttt{You are CompareGPT, a machine to verify the correctness of predictions. Answer with only yes/no. You are given a question, the corresponding ground-truth answer and a prediction from a model. Compare the "Ground-truth answer" and the "Prediction" to determine whether the prediction correctly answers the question. All information in the ground-truth answer must be present in the prediction, including numbers and dates. You must answer "no" if there are any specific details in the ground-truth answer that are not mentioned in the prediction. There should be no contradicting statements in the prediction. The prediction may contain extra information. If the prediction states something as a possibility, treat it as a definitive answer.}\\
% \midrule
% \textbf{Instruction 4}\\
% \midrule
% \texttt{You are CompareGPT, a machine to verify the groundedness of predictions. Answer with only yes/no. You are given a question, the corresponding evidence and a prediction from a model. Compare the "Prediction" and the "Evidence" to determine whether all the information of the prediction in present in the evidence or can be inferred from the evidence. You must answer "no" if there are any specific details in the prediction that are not mentioned in the evidence or cannot be inferred from the evidence.}\\
\bottomrule
\end{tabular}
\caption{All prompt instructions}
\label{fig:prompts}
\end{figure}

==> Figures/unanswerability_manual_inspection.tex <==
\begin{figure*}[ht!]
\small
\begin{tabular}{p{2\columnwidth}}
\toprule

\textbf{Dataset}: NQ \\
\\
\textbf{Question}: points on a sphere or angles in a circle are measured in units called \\
\textbf{Reference answer}: radians\\
\textbf{Responses}:\\ 
\textbf{Alpaca}: \textcolor{purple}{radians}\\
\textbf{Flan-T5}: \textcolor{teal}{I don't know}\\
\textbf{GPT-3.5}: \textcolor{purple}{degrees}\\
\colorbox{red!10}{\textbf{Irrelevant knowledge}:} Title: Inscribed angle\\
inscribed angle theorem states that an angle $\theta$ inscribed in a circle is half of the central angle 2$\theta$ that subtends the same arc on the circle. Therefore, the angle does not change as its vertex is moved to different positions on the circle...
\\
\midrule
\textbf{Question}: who played the colorado kid in rio bravo \\
\textbf{Reference answer}: Ricky Nelson\\
\textbf{Responses}: \\
\textbf{Alpaca}: \textcolor{purple}{The role of the Colorado Kid was played by John Dehner in the 1959 film Rio Bravo.}\\
\textbf{Flan-T5}: \textcolor{purple}{Jim J. Bullock}\\
\textbf{GPT-3.5}: \textcolor{teal}{I don't know.}\\
\colorbox{red!10}{\textbf{Irrelevant knowledge}:} Title: Jim J. Bullock\\
Jim J. Bullock James Jackson Bullock (born February 9, 1955), sometimes credited as Jm J. Bullock, is an American actor and comedian of stage, television and motion pictures... Bullock became a notable entertainment figure in the 1980s \\
\midrule

\textbf{Dataset}: HotpotQA \\
\\
% \textbf{Question}: Are both Elko Regional Airport and Gerald R. Ford International Airport located in Michigan?  \\
% \textbf{Reference answer}: no\\
% \textbf{Responses}:\\ 
% \textbf{Alpaca}: \textcolor{purple}{No, Elko Regional Airport is located in Elko, Nevada, and Gerald R. Ford International Airport is located in Grand Rapids, Michigan.}\\
% \textbf{Flan-T5}: \textcolor{purple}{no}\\
% \textbf{GPT-3.5}: \textcolor{teal}{I don't know}\\
% \colorbox{red!10}{\textbf{Irrelevant knowledge}:} Title: Elwood Airport\\
% Elwood Airport (FAA LID: 3I1) was a public use airport located two nautical miles (3.7km) south of the central business district of Elwood, in Madison County, Indiana, United States. The airfield closed on September 1, 2008.
% \\
% \midrule
\textbf{Question}: Ralph Hefferline was a psychology professor at a university that is located in what city? \\
\textbf{Reference answer}: New York City\\
\textbf{Responses}: \\
\textbf{Alpaca}: \textcolor{purple}{Columbia, Missouri.}\\
\textbf{Flan-T5}: \textcolor{purple}{Columbia}\\
\textbf{GPT-3.5}: \textcolor{teal}{I don't know.}\\
\colorbox{red!10}{\textbf{Irrelevant knowledge}:} Title: University of Missouri\\
The University of Missouri (also, Mizzou, or MU) is a public land-grant research university located in Columbia, Missouri, U.S. It was founded in 1839 ...
\\
\midrule
\textbf{Dataset}: TopiOCQA \\
\\
% \textbf{Question}: \\
% User: where may have the mycenaeans ultimately ended up\\
% Agent: Cyprus and the Levantine coast\\
% User: where is the former place located?\\
% \textbf{Reference answer}: In the Eastern Mediterranean, located south of Turkey; west of Syria and Lebanon; north of Egypt, Israel, and Palestine; and southeast of Greece.\\
% \textbf{Responses}:\\ 
% \textbf{Alpaca}: \textcolor{purple}{Cyprus is located in the Mediterranean Sea, south of Turkey, west of Syria and Lebanon, and north of Egypt.
% }\\
% \textbf{Flan-T5}: \textcolor{purple}{Cyprus}\\
% \textbf{GPT-3.5}: \textcolor{teal}{I don't know.}\\
% \colorbox{red!10}{\textbf{Irrelevant knowledge}:} Title: Ancient history of Cyprus\\
% Cyprus became a Roman province in 58 BCE. This came about, according to Strabo, because Publius Clodius Pulcher held a grudge against Ptolemy of Cyprus...
% \\
% \midrule
\textbf{Question}: \\
User: what is the location of mars in the solar system\\
Agent: Mars is the fourth planet from the Sun\\
User: is it known by any other names? \\
\textbf{Reference answer}: Red Planet\\
\textbf{Responses}: \\
\textbf{Alpaca}: \textcolor{purple}{No, it is known by its official name, Mars.}\\
\textbf{Flan-T5}: \textcolor{purple}{Mars is also known as the Red Planet.}\\
\textbf{GPT-3.5}: \textcolor{teal}{I don't know.}\\
\colorbox{red!10}{\textbf{Irrelevant knowledge}:} Title: Haboob\\
Global dust storms on Mars have been compared to haboobs on Earth.
\\
\bottomrule
\end{tabular}
\caption{Failure examples of the models in generating \emph{I don't know} in the presence of irrelevant knowledge.}\label{fig:unanswerability_irrelevant}
\end{figure*}


\begin{figure*}[ht!]
\small
\begin{tabular}{p{2\columnwidth}}
\toprule

\textbf{Dataset}: NQ \\
\\
\textbf{Question}: points on a sphere or angles in a circle are measured in units called \\
\textbf{Reference answer}: radians\\
\textbf{Responses}:\\ 
\textbf{Alpaca}: 1. \textcolor{teal}{radians}\\
\textbf{Flan-T5}: \textcolor{teal}{radians}\\
\textbf{GPT-3.5}: \textcolor{purple}{I don't know.}\\
\colorbox{green!10}{\textbf{Relevant knowledge}:} Title: Position angle\\
... It is calculated in a plane that contains the sphere center and the great circle, where is the angular distance of two points viewed from the center of the sphere, measured in \textbf{radians}...
\\
\midrule
\textbf{Question}: who had a baby at 100 in the bible \\
\textbf{Reference answer}: 1. Sarah, 2. Abraham\\
\textbf{Responses}:\\ 
\textbf{Alpaca}: 100 year old \textcolor{teal}{Sarah} had a baby with \textcolor{teal}{Abraham}.\\
\textbf{Flan-T5}: \textcolor{purple}{I don't know.}\\
\textbf{GPT-3.5}: \textcolor{teal}{Abraham} had a baby at 100 in the Bible.\\
\colorbox{green!10}{\textbf{Relevant knowledge}:} Title: The Bible and humor\\
... Macy says that in speaking of humor in the Bible he usually begins with asking how it might feel to personally get the message \textbf{Abraham and Sarah} received, putting them into the absurd situation of \textbf{a ninety year old having a baby}...
\\
\midrule

% \textbf{Question}: when did the isle of wight become an island \\
% \textbf{Reference answer}: During the last Ice Age\\
% \textbf{Responses}: \\
% \textbf{Alpaca}: 11,755 years ago, \textcolor{teal}{during the last ice age}, forming the Solent and turning Wight into an island. The Needles, along with Old Harry Rocks on Purbeck, represent the edges of this breach.\\
% \textbf{Flan-T5}: \textcolor{teal}{during the last ice age
% }\\
% \textbf{GPT-3.5}: \textcolor{purple}{I don't know.}\\
% \colorbox{green!10}{\textbf{Relevant knowledge}:} Title: Isle of Wight\\
% \textbf{during the last ice age}, forming the Solent and turning Wight into an island. The Needles, along with Old Harry Rocks on Purbeck, represent the edges of this breach...
% \\
% \toprule

\textbf{Dataset}: HotpotQA \\
\\
% \textbf{Question}: Are the Laleli Mosque and Esma Sultan Mansion located in the same neighborhood? \\
% \textbf{Reference answer}: no\\
% \textbf{Responses}:\\ 
% \textbf{Alpaca}: \textcolor{teal}{No}, they are not. The Laleli Mosque is located in the Fatih neighborhood of Istanbul, while the Esma Sultan Mansion is located in the Ortaköy\\
% \textbf{Flan-T5}: \textcolor{teal}{no}\\
% \textbf{GPT-3.5}: \textcolor{purple}{I don't know}\\
% \colorbox{green!10}{\textbf{Relevant knowledge}:} \\
% - Title: Laleli Mosque\\
% The Laleli Mosque (Turkish: "Laleli Camii, or Tulip Mosque" ) is an 18th-century Ottoman imperial mosque located in \textbf{Laleli, Fatih}, Istanbul, Turkey.\\
% - Title: Esma Sultan Mansion\\
% The Esma Sultan Mansion (Turkish: "Esma Sultan Yalısı" ), a historical yalı (English: waterside mansion ) located at Bosphorus in \textbf{Ortaköy neighborhood} of Istanbul, Turkey...
% \\
% \midrule
\textbf{Question}: Roger O. Egeberg was Assistant Secretary for Health and Scientific Affairs during the administration of a president that served during what years? \\
\textbf{Reference answer}: 1969 until 1974\\
\textbf{Responses}: \\
\textbf{Alpaca}: \textcolor{teal}{1969-1974.}\\
\textbf{Flan-T5}: \textcolor{teal}{1969 until 1974.}\\
\textbf{GPT-3.5}: \textcolor{purple}{I don't know.}\\
\colorbox{green!10}{\textbf{Relevant knowledge}:} \\
Title: Roger O. Egeberg\\
... His other roles included Assistant Secretary for Health and Scientific Affairs in the Department of Health, Education, and Welfare (now the United States Department of Health and Human Services) during the \textbf{Nixon administration} and Dean of the University of Southern California's medical school.\\
- Title: Richard Nixon\\
Richard Milhous Nixon (January 9, 1913 – April 22, 1994) was the 37th President of the United States \textbf{from 1969 until 1974}, ...\\
\midrule
\textbf{Dataset}: TopiOCQA \\
\\
% \textbf{Question}: \\
% User: where may have the mycenaeans ultimately ended up\\
% \textbf{Reference answer}: Cyprus and the Levantine coast\\
% \textbf{Responses}:\\ 
% \textbf{Alpaca}: The Mycenaeans ultimately ended up in a number of different places, including the Aegean islands, the Peloponnese, \textcolor{teal}{Cyprus, and the Levantine coast.}\\
% \textbf{Flan-T5}: Mycenaean refugees migrated to \textcolor{teal}{Cyprus and the Levantine coast.}\\
% \textbf{GPT-3.5}: \textcolor{purple}{I don't know.}\\
% \colorbox{green!10}{\textbf{Relevant knowledge}:} Title: Mycenaean Greece\\
% Mycenaean refugees migrated to Cyprus and the Levantine coast. Nevertheless, other regions on the edge of the Mycenaean world prospered, such as the Ionian islands, the northwestern Peloponnese, parts of Attica and a number of Aegean islands. The acropolis of Athens, oddly, appears to have avoided destruction.
% \\
% \midrule
\textbf{Question}: \\
User: how much did the blues brothers movie cost to make\\
\textbf{Reference answer}: \$17.5 million\\
\textbf{Responses}: \\
\textbf{Alpaca}: \textcolor{teal}{17.5 million}\\
\textbf{Flan-T5}: \textcolor{teal}{\$17.5 million}\\
\textbf{GPT-3.5}: \textcolor{purple}{I don't know.}\\
\colorbox{green!10}{\textbf{Relevant knowledge}:} Title: The Blues Brothers (film)\\
Principal photography began in July 1979, with the film's budget still not settled. For the first month, things ran smoothly on and off the set. When Weiss saw the supposedly final \textbf{\$17.5 million} budget, he reportedly joked, "I think we've spent that much already." ...
\\
\bottomrule
\end{tabular}
\caption{Failure examples of the models in generating informative responses in the presence of relevant knowledge.}\label{fig:unanswerability_relevant}
\end{figure*}

==> Figures/unanswerability_manual_inspection_numerous_examples.tex <==
\begin{figure*}[ht!]
\small
\begin{tabular}{p{2\columnwidth}}
\toprule
% \textbf{Error Type:} More Elaborate Answers\\
% \textbf{Dataset}: HotpotQA \\
% \\
% \textbf{Question}: At what theater is the composer and lyricist for the musical Big Fish a residential artist? \\
% \textbf{Reference answer}: Ars Nova Theater \\
% \textbf{Model response (Alpaca)}: The composer and lyricist for the musical Big Fish, Andrew Lippa, is a residential artist at the Ars Nova Theater in New York City.\\
% \\
% \textbf{Scores}: \\F1: 26.0, Recall: 100.0, BLEU: 0, METEOR: 54.5, Rouge-L: 22.2, BertS (F1): 85.4, BEM: 98.9, GPT4-Eval: 100.0\\
% \midrule
% \textbf{Error Type:} Open-ended Questions\\
% \textbf{Dataset}: TopiOCQA \\
% \\
% \textbf{Question}: what was the watergate scandal? \\
% \textbf{Reference answer}: It was an array of clandestine and often illegal activities undertaken by members of the Nixon administration. \\
% \textbf{Model response (Flan-T5)}: The Watergate scandal was a political scandal in the United States involving the administration of U.S. President Richard Nixon from 1972 to 1974 that led to Nixon's resignation.\\
% \\
% \textbf{Scores}: \\F1: 21.8, Recall: 26.7, BLEU: 0, METEOR: 15.6, Rouge-L: 15.4, BertS (F1): 86.1, BEM: 73.9, GPT4-Eval: 100.0\\
% \midrule
% \textbf{Error Type:} Enumeration of reference answers\\
\textbf{Dataset}: NQ \\
\\
\textbf{Question}: points on a sphere or angles in a circle are measured in units called \\
\textbf{Reference answer}: radians\\
\textbf{Model response (GPT-3.5)}: \colorbox{orange!10}{I don't know.}\\
\colorbox{green!10}{\textbf{Correct Passage}:} Title: Position angle \\
... It is calculated in a plane that contains the sphere center and the great circle, where is the angular distance of two points viewed from the center of the sphere, \textbf{measured in radians}... 
\\
\midrule
\textbf{Question}: who is the biggest selling female group of all time  \\
\textbf{Reference answer}: Spice Girls\\
\textbf{Model response (Flan-T5)}: \colorbox{orange!10}{I don't know}\\
\colorbox{green!10}{\textbf{Correct Passage}:} Title: Spice Girls\\
... In total, the album sold over 3 million copies in Britain, \textbf{the biggest-selling album of all time in the UK by a female group}, certified 10× Platinum, and peaked at number one for fifteen non-consecutive weeks.
\\
\midrule
\textbf{Question}: factories that assemble parts made in other countries  \\
\textbf{Reference answer}: special economic zones\\
\textbf{Model response (Alpaca-7B)}: \colorbox{orange!10}{1. Yes 2. No 3. I don't know}\\
\colorbox{red!10}{\textbf{Incorrect Passage}:} Title: Antonio Marcegaglia\\
... The expansion of its industrial activities continued in 2008 with its entry into China, where, in Yangzhou, 350 km north-west of Shanghai, it created its first Asian plant for the production of stainless steel tubes and high-precision carbon steel ... 
\\
\toprule
\textbf{Dataset}: HotpotQA \\
\\
\textbf{Question}: Roger O. Egeberg was Assistant Secretary for Health and Scientific Affairs during the administration of a president that served during what years? \\
\textbf{Reference answer}: 1969 until 1974\\
\textbf{Model response (GPT-3.5)}: \colorbox{orange!10}{I don't know.}\\
\colorbox{green!10}{\textbf{Correct Passages}:} \\
- Title: Roger O. Egeberg\\
... His other roles included Assistant Secretary for Health and Scientific Affairs in the Department of Health, Education, and Welfare (now the United States Department of Health and Human Services) \textbf{during the Nixon administration} ... \\
- Title: Richard Nixon\\
Richard Milhous Nixon (January 9, 1913 – April 22, 1994) was the 37th President of the United States \textbf{from 1969 until 1974} ...\\
\midrule
\textbf{Question}: Although a dependent territory remains politically outside of the controlling state's integral area, what else can it contain? \\
\textbf{Reference answer}: the flags\\
\textbf{Model response (Flan-T5)}: \colorbox{orange!10}{I don't know}\\
\colorbox{green!10}{\textbf{Correct Passages}:} \\
- Title: Gallery of flags of dependent territories\\
This overview contains \textbf{the flags of dependent territories} and other areas of special sovereignty...\\
- Title: Dependent territory\\
A dependent territory, dependent area or dependency is a territory that does not possess full political independence or sovereignty as a sovereign state yet remains politically outside of the controlling state's integral area.\\
\midrule
\textbf{Question}: Insomniac Events is part of a partnership with a club founded by an investor of what heritage?  \\
\textbf{Reference answer}: Iranian-American\\
\textbf{Model response (Alpaca-7B)}: \colorbox{orange!10}{I don't know.}\\
\colorbox{green!10}{\textbf{Correct Passages}:} \\
- Title: Insomniac Events\\
... Insomniac is involved in the operation of three Los Angeles nightclubs - Create (in partnership with \textbf{SBE}, built on the site of the former Vanguard Hollywood), Exchange L.A. and the underground warehouse Factory 93, located at 1756 Naud Street...\\
- Title: Sam Nazarian\\
Sam Nazarian (born 1975) is \textbf{an Iranian-American businessman}, investor and philanthropist. He is \textbf{the Founder, Chairman and CEO of SBE Entertainment Group}.\\
\toprule
\textbf{Dataset}: TopiOCQA \\
\\
\textbf{Question}: how much did the blues brothers movie cost to make \\
\textbf{Reference answer}: More than \$17.5 million\\
\textbf{Model response (GPT-3.5)}: \colorbox{orange!10}{I don't know.}\\
\colorbox{green!10}{\textbf{Correct Passage}:} Title: The Blues Brothers (film)\\
... For the first month, things ran smoothly on and off the set. When Weiss saw the supposedly final \textbf{\$17.5 million budget}, he reportedly joked, "I think we've spent that much already." ...\\
\midrule
\textbf{Question}: how much did the blues brothers movie cost to make \\
\textbf{Reference answer}: 1. A high-pressure area, high ,or anticyclone, 2. High-pressure systems rotate clockwise in the northern Hemisphere, 3. UNANSWERABLE, 4. Referred as anticyclones\\
\textbf{Model response (Flan-T5)}: \colorbox{orange!10}{I don't know}\\
\colorbox{green!10}{\textbf{Correct Passage}:} Title: High-pressure area\\
A high-pressure area, high, or anticyclone, is a region where the atmospheric pressure at the surface of the planet is greater than its surrounding environment...\\
\bottomrule
\end{tabular}
\caption{Failure examples of the models in generating \emph{I don't know} with or without presence of gold passage}
\end{figure*}

==> Sections/_results.tex <==
\section{Results and Discussion}
{\color{red}TODO: write summary after completing this section}
% In this section, we report the impact of instruction-tuning with demonstrating some of the failure cases. 
\subsection{Experimental Setup}
In our experiments, we provide 10 top retrieved passages to the generative model and use 0.95 for \texttt{temperature} and \texttt{top\_p} and 50 as the maximum number of generated tokens.
\subsection{What is the impact of instruction-tuning? (Q1)}
We compare the performance of OPT~\cite{zhang2022opt} and Llama~\cite{touvron2023llama} with the instruction-tuned models OPT-IML~\cite{iyer2023optiml} and Alpaca~\cite{Taori2023alpaca} in \Cref{?}. These results show that instruction-tuning affects the performance significantly in all studied datasets. Although these models have probably seen NaturalQuestions and HotpotQA samples during the tuning phase, we hypothesize that TopiOCQA hasn't been used for instruction-tuning of these models. 

\textcolor{\commentcolor}{<Plot for llama vs. alpaca and opt vs. opt-iml>}

The performance of different retrieval-augmented QA models is presented in \Cref{?}. The results demonstrate that, overall, Flan-T5-xxl and OPT-iml perform the best, while the former is superior. 

\textcolor{\commentcolor}{<Plot for all instruction-tuned together with the model size - with the same retriever>}

\begin{table*}[h]
    \centering
    \begin{tabular}{m{5cm}|m{5cm}|m{5cm}}
        \multicolumn{3}{c}{Question: Which mountain is located in China, Kirat Chuli or Kangpenqing?} \\
        \multicolumn{1}{c}{BM25} & \multicolumn{1}{c}{DPR} & \multicolumn{1}{c}{Contriever} \\\hline
        \begin{tabular}{@{}m{5cm}@{}}
        - Kirat Chuli | \textbf{Kirat Chuli} or Tent Peak is a mountain in the Himalayas.\\
        - Kangpenqing | \textbf{Kangpenqing} is a mountain in the Baiku Himalayas of Tibet, China.\\
        - World altitude record | ... On 24 May he solo-climbed Nepal Peak near \textbf{Kirat Chuli}.
        \end{tabular} &
        \begin{tabular}{@{}m{5cm}@{}}
        - Kirat Chuli | \textbf{Kirat Chuli} or Tent Peak is a mountain in the Himalayas.\\[80pt]
        \end{tabular} 
        &
        \begin{tabular}{@{}m{5cm}@{}}
        - Kangpenqing | \textbf{Kangpenqing} is a mountain in the Baiku Himalayas of Tibet, China.\\
        - Kangchenjunga | ... The northern section includes Yalung Kang, Kangchenjunga Central and South, Kangbachen, \textbf{Kirat Chuli}, etc.
        \end{tabular}
    \end{tabular}
    \caption{The retrieved passages for a multichoice question in HotpotQA. Unlike passages retrieved by DPR and Contriever, the passages retrieved by BM25 perfectly describe the two choices \textit{Kirat Chuli} and \textit{Kangpenqing}. The passages are shortened due to space limits.}
    \label{tab:retriever_multichoice_failure}
\end{table*}

Furthermore, \Cref{?} shows the retriever's contribution to the overall performance. It can be observed that sparse retrievers (e.g., BM25) are more useful on HotpotQA and dense retrievers (e.g., DPR and Contriever) perform better on NaturalQuestions. We hypothesize that this is because in many of the multichoice samples in HotpotQA, the top retrieved passages of dense retrievers do not cover the best existing passages about all the options. However, with sparse retrievers, passages with more lexical overlap are retrieved. This phenomenon is illustrated in \Cref{tab:retriever_multichoice_failure}.

\textcolor{\commentcolor}{<Plot for all retrievers - with the same generator>}

\subsection{Do current metrics represent the models' failures? (Q2)}
There are a couple of reasons why a generated response by large instruction-tuned models does not achieve a perfect score. The main reasons observed in the experiments are as follows:

\textcolor{\commentcolor}{<A Plot or a table showing the \% each incorrect answer belongs to the failure cases. If there are a lot of them in verbosity and formatting, then we can better make a claim that metrics are not good enough ... >} 
\begin{itemize}
    \item Incorrect generation, where the model generates an incorrect response, while the correct answer appears in the context.

    \item \textcolor{\commentcolor}{not sure:} Distracting or incorrect retrieval, where the generated response is truly incorrect because the retrieved context not only doesn't include the correct answer but also provides some distracting information.

    \item \textcolor{\commentcolor}{not sure:} Hallucination, where the model generates a factually incorrect response that is not included in the context.

    \item Requiring clarification, which mostly happens with large GPT models, where the model asks for further information or clarification when the answer does not appear in the context.
    
    \item Formatting, where the generated response is in fact correct, but does not match the specific formatting of the gold answer. This mostly happens with dates, middle names, etc.

    \item Verbosity, where the generated answer is technically correct but the model elaborates more on the response. This problem mostly happens using GPT models.

\end{itemize}
\textcolor{\commentcolor}{A table with examples of each reason in each row, and the F1 or Exact match score in the next columns, that shows how current responses get very low scores.}

\subsection{Instruction-tuned models vs. Finetuned models? (Q3)}
When it comes to intruction-tuned models, an important challenge is to decide to use whether an instruction-tuned model or a model specifically finetuned on the target dataset. In this section, we compare the performance of popular finetuned models on our studied datasets.
\textcolor{\commentcolor}{I think it is better to first mention the problem with metrics, and then talk about this. Because using Recall scores, we can better claim that instruction-tuned models are performing reasonably well compared to finetuned models (we don't have recall for Atlas on NQ, but this is the case with recall score on TopiOCQA.)}

\subsection{Are instruction-tuned models faithful?}

% {
% \color{\commentcolor}
% Plots:
% \begin{itemize}
%     \item instruction-tuned vs. non-intruction-tuned (llama vs. alpaca, opt vs. opt-iml)\label{fig:results:instruction_vs_non_instruction}
%     \item all instruction-tuned together\label{fig:results:all_instruction}
%     \item instruction-tuned vs. finetuned (on NQ, TopiOCQA)\label{fig:results:instruction_vs_finetune}
% \end{itemize}
% }



==> Sections/all_results_compilation.tex <==
\section{Multi-faceted Evaluation of Instruction-following Models for QA}



% Equipped with insights about how to evaluate instruction-following models, we present the results for correctness w.r.t information need (\Cref{tab:main_results_correctness}) and faithfulness w.r.t provided knowledge (\Cref{tab:main_results_faithfulness}). Based on these results, we answer the following research questions. \\
\iffalse
\noindent\textit{Do current instruction-following models outperform fine-tuned models for correctness?}

\noindent To compare against instruction-following models, we select FiD \cite{izacard2021fid} as our fine-tuned baseline for all three tasks. For NQ and TopiOCQA, we use the publicly available FiD checkpoints. For HotpotQA, we fine-tune our own variant using the default hyperparameters.

Unlike instruction-following models (\Cref{sec:retrieval}), FiD is not restricted by input context size for the number of retrieved passages. We use the default settings for each dataset -- 100 passages for NQ, 50 passages for TopiOCQA, and up to 18 passages for HotpotQA. For HotpotQA, the top 100 reasoning chains produced by the retriever are de-duplicated to generate the final passage set.


In \Cref{tab:main_results_correctness}, we report EM, F1, and Recall for assessing correctness. Unsurprisingly, FiD scored higher than instruction-following models on traditional QA metrics like EM and F1 (with the exception of Flan-T5 on HotpotQA). However, based on our findings (\Cref{sec:correctness}), we rely on Recall for a more accurate performance measure. Using recall, the performance gap narrows significantly, with some instruction-following models even outperforming fine-tuned FiD. Notably, GPT-3.5 outperforms FiD across all three QA tasks -- by 6.48\% in NQ, 10.27\% in HotpotQA, and 9.33\% in TopiOCQA, whereas Llama-2 outperforms FiD on two out of three tasks and matches FiD's performance in TopiOCQA. Overall, these results suggest that in retrieval-augmented settings, instruction-following models are equally, or even more capable than fine-tuned generators in generating correct responses w.r.t user information needs.

It is worth noting that although some model training includes NQ and HotpotQA, TopiOCQA serves as a true test of zero-shot generalization. TopiOCQA is not included in any instruction-tuning datasets and was released after the knowledge cutoff of GPT-3.5 (September 2021). \\

\noindent\textit{Are instruction-following models faithful w.r.t relevant knowledge?}

\noindent For faithfulness w.r.t relevant knowledge, we report K-F1 and K-Precision in \Cref{tab:main_results_faithfulness}. According to K-F1, which is typically used in the literature, Llama-2 is the most grounded in the provided relevant knowledge, closely followed by GPT-3.5, whereas Flan-T5 is consistently ranked the lowest.

On the other hand, K-Precision, the metric most correlated with human judgments (\Cref{sec:groundedness_gold_passage}), denotes a completely different trend. GPT-3.5 is the \emph{least} faithful for NQ, while Llama-2 is the least faithful for HotpotQA and TopiOCQA. Flan-T5 achieves the highest score for all three tasks, outperforming all others by a significant margin.
% As K-F1 rewards equivalence between the provided passage and the model response, it unfairly penalizes the short responses of Flan-T5, when compared to a much longer knowledge snippet.
The stark difference between the scores of Flan-T5 and other models also denotes a trade-off between correctness and faithfulness -- GPT-3.5 and Llama-2 outperform Flan-T5 in correctness but lag behind significantly in faithfulness. \\

\noindent\textit{How well can models follow the input instruction?}

\noindent To evaluate models for faithfulness w.r.t irrelevant knowledge, we provide explicit instruction to the model to output ``I don’t know'' when an irrelevant passage is provided (\Cref{sec:unanswerability}). We report the proportion of responses in which the model refused to answer in \Cref{tab:main_results_faithfulness}. GPT-3.5 most often refrains from answering when given an irrelevant passage (98\% in NQ and HotpotQA, 88\% in TopiOCQA), followed closely by Llama-2.

However, just based on providing an irrelevant passage, it is unclear whether the models actually judged the relevance of the passage or just defaulted to saying ``I don't know''. When provided with a gold passage with the same instruction, both the models still often chose not to answer, with Llama-2 refusing more than 50\% of the time across all datasets. Flan-T5, which appears relatively well-balanced, remains overconfident on TopiOCQA (which was not included in its training), refraining from answering only 40\% of times when provided with irrelevant passage. Alpaca adheres the least to the instruction and refrains from answering only 0-2\% of times in either scenario. Overall, the results indicate that further research is required to optimally design and prompt models to better identify when to refrain from answering.
\fi

Additionally, we also investigate the impact of input instruction on correctness w.r.t information need. We provide the models with the instruction from \Cref{sec:unanswerability} in the retrieval-augmented setting and compare the results to the original setup (\Cref{tab:main_results_correctness}).
% (i.e. when the input instruction \textit{does not} explicitly instruct the model to refrain from answering).

GPT-3.5 and Llama-2 suffer a significant loss in performance due to changes in the instruction. For example, the recall of GPT-3.5 dropped from 57.98 to 34.1 on NQ. Overall, GPT-3.5 experienced a 37.26\% performance drop across all three datasets, while Llama-2 faced 29.37\%. In contrast, Flan-T5 and Alpaca are relatively less affected, with only 5.06\% and 1.04\% drop respectively. It is possible that GPT-3.5 and Llama-2, both of which are trained using RLHF, might lean more towards refraining from answering to avoid providing misinformation, especially when an explicit instruction to do so is present.



% \input{Tables/prompt_sensitivity}

% \noindent\textit{Are instruction-following models sensitive to the input prompt?}

% How well can models follow the input instruction





==> Sections/datasets.tex <==
\subsection{Data}


\paragraph{Open Squad}


\paragraph{HotPotQA:}
% full wiki setting

\paragraph{Natural Questions:}



\paragraph{TopiOCQA:} 



\paragraph{FaithDial}

==> Sections/discussion.tex <==
\section{Discussion and Limitations}
\label{sec:discussion}
Below, we highlight several key findings of this paper and  discuss some 
 of its limitations.

\paragraph{Evaluation Metrics}
Our analysis demonstrates that widely used metrics are not suitable for evaluating correctness and faithfulness.
We propose that Recall and K-Precision as widely accessible and human-aligned metrics for correctness and faithfulness, however, we emphasize that these simple lexical-based metrics are easy to hack. One model can copy all the retrieved knowledge as the output, leading to high Recall and K-Precision metrics. However, such a model will be penalized heavily when evaluated for faithfulness w.r.t. irrelevant knowledge.

\paragraph{Instruction-Following Models}
According to the most human aligned and easy to use metrics (i.e., Recall and K-Precision), we conclude that GPT-3.5 outperforms other models on majority of the datasets in correctness w.r.t information need. However, when analyzing the faithfulness w.r.t relevant knowledge, Flan-T5 is shown to be the best model in all three datasets. 
Moreover, our further analysis on the models' faithfulness w.r.t irrelevant knowledge demonstrates that models struggle to correctly identify whether the provided knowledge is relevant or not.


% although Flan-T5 is well balanced on datasets it was exposed to during training, it remains overconfident on TopiOCQA, which was not included in
% the training. While GPT-3.5 is shown
% to be overly cautious, refraining to answer 26-49\% of the time given correct knowledge, Alpaca almost always responds with an answer, almost never outputing “I don’t know” in its response. 
\paragraph{Limitations}
It is worth mentioning that 
% % The followings are mentioned in the "Limitations"
% these observations are based on the performance of the models in a zero-shot setting, without exhaustive prompt engineering. Furthermore, 
the experiments for evaluating the faithfulness of the models are conducted in a modified setting, where a relevant or irrelevant passage is provided in the prompt on purpose. This is different from the real-world scenario, where the retrieved passages can contain a mix of relevant and irrelevant knowledge.

Finally, it should also be noted that beyond
qualitative investigation, we did not explore a wide range of prompts for the tasks studied in this work. Recent work has shown that the performance of instruction-following models can vary greatly depending upon the provided prompt \citep{zhao2021calibrate,liu_prompting_2021}. We leave it to future works to investigate better prompts for instruction-following models in a retrieval-augmented setting.

\ignore{
\paragraph{Limitations}
We describe the main limitations of our work below.

\noindent
\textbf{1) We did not extensively explore prompts for instruction-following models.}
Recent work has shown that the performance of instruction-following models can vary greatly depending upon the provided prompt \citep{zhao2021calibrate,liu_prompting_2021}.
Beyond qualitative investigation, we did not explore a wide range of prompts for the tasks studied in this work.
For example, better prompts may exist for eliciting more grounded model responses.
Future work can investigate better prompts for instruction-following models in a retrieval-augmented setting.


\noindent
\textbf{2) We only evaluate models in a \emph{zero-shot} setting.}
Recent work has shown that instruction-following models can leverage in-context demonstrations to improve performance on a variety of NLP tasks \citep{brown2020gpt,du_glam_2021,rae_scaling_2022}.
While these performance increases carry additional computational cost \citep{liu_few-shot_2022}, particularily in a retrieval-augmented setting, future work can investigate the performance of instruction-following models for QA in a few-shot setting.


\noindent
\textbf{3) Biases may exist within our human evaluation setup.}
Most importantly, all annotations within this paper were done by the four graduate student authors.
Additionally, we only annotated a small subset of examples from each dataset.
While we took steps to attempt to mitigate any annotation biases (e.g., blind review of model responses), biases likely exist in our evaluation.
}

% \todo{VA: a trend of more correct models are less faithful}
% \paragraph{Finding better metrics to evaluate correctness}
% Regarding the correctness of model responses, we find that, among annotations marking a model as correct, there are close to 300 instances where $\text{F1}<0.3$.
% Upon further investigations (\Cref{sec:correctness_results}), we observe that a majority of errors are caused by the use of more elaborate answers, followed by answers differing due to open-ended questions (see \Cref{fig:correctness_error_analysis}).
% This is illustrated in \Cref{fig:manual_inspection}, where we see that F1 is low when the model reiterates the question, provides an alternative but correct response, or lists all the reference answers. 

% Clearly, F1 is not a suitable metric for instruction-following models, missing obviously correct answers.
% This leads to the question: which metric among the ones introduced in \Cref{sec:correctness_metrics} would be better?
% To find out, we correlate them with human judgement (\Cref{tab:correctness_human_correlations}) and find that Recall and GPT4-Eval are the best lexical and model-based metrics, respectively.
% Although they have a 8-12 points difference, the latter is slow to run, expensive, and difficult to reproduce.
% Thus, using Recall (which achieves a moderate correlation), we find that GPT-3.5 outperforms other instruction-following models (as well as the finetuned FiD) in 2 out of 3 tasks (\Cref{tab:correctness_main_results}) on the recall metric, but significantly underperforms on all lexical metrics, as well as the popular BERTScore. 

% \paragraph{Evaluating faithfulness requires other metrics}
% % Similar to the analysis on correctness of the models, we find that K-Precision and LLMCritic (GPT-4) give us a fair estimate of the models' faithfulness in a given QA task as they outperform other studied metrics (\Cref{tab:overall_correlations_faithfulness}). Considering K-Precision as the cheapest and easiest metric to evaluate the models on all the datasets, we find in \Cref{tab:faithfulness_table} that ...
% It would be tempting, based on the results mentioned above, to directly extend promising metrics like Recall or GPT3.5-Eval to evaluate model faithfulness; after all, retrieved passages are directly related to the reference answers for the three QA tasks.
% It may therefore be counter-intuitive to observe, in \Cref{tab:overall_correlations_faithfulness}, that knowledge-based precision is more correlated with human judgement compared to K-Recall, and that LLMCritic (GPT-3.5) lags behind K-Precision and the larger GPT-4 variant.
% Based on the assumpution that K-Precision can give us a fair estimate of a model's faithfulness in a given QA task, we find in \Cref{tab:faithfulness_table} that GPT-3.5 is less faithful than Flan-T5, which has seen instructions sourced from NQ\footnote{\href{https://github.com/allenai/natural-instructions/pull/278}{github.com/allenai/natural-instructions/pull/278}} and HotpotQA\footnote{\href{https://github.com/allenai/natural-instructions/pull/107}{github.com/allenai/natural-instructions/pull/107}}.
% However, this is not supported by a strong correlation, as automatic faithfulness metrics are much less correlated with human judgement compared to correctness metrics.

% \paragraph{Models struggle with responding ``I don't know'' given irrelevant knowledge}
% At this point, we know that one model is better at providing a good response (w.r.t. reference answers) whereas another is more grounded to the provided passage.
% However, we have been assuming that the provided passage is itself correct.
% This is unfortunately not always the case, and when an incorrect passage is provided, a good generator should refuse to answer.
% To this end, we explore in \Cref{sec:unanswerability} a simple change in the prompt (i.e. by prompting the model to output ``I don't know'' when the provided passage is not useful).
% In \Cref{tab:unanswerability}, we find that GPT-3.5 is overly cautious, outputting ``I don't know'' 26-49\% of the time when the provided passage contains the answer, whereas Alpaca simply ignores this new instruction, as it almost never output ``I don't know'' in its response.
% Although Flan-T5 is well balanced on datasets it was exposed to during training, it remains overconfident on TopiOCQA, which was not included in the training tasks.

% \paragraph{Recommendations for correctness, faithfulness, and beyond}
% Based on those results, we recommend the use of recall or specialized model-based metrics when evaluating on NQ, HotpotQA and TopiOCQA to determine if a response is correct based on reference answers.
% For other datasets (or models significantly different from evaluated ones), careful human evaluation should be performed to uncover possible issues with traditional metrics and find the most correlated metric among a diverse pool of metrics, both lexical and model-based.
% We also suggest, as future work, to develop better metrics for evaluating faithfulness of instruction-following models that better reflect human judgement, and improve current approaches for correctness.
% To this end, we will release our user interface and annotations for the research community to build-upon, as well as relevant source code to reproduce our RAG evaluation experiments.

==> Tables/correctness_results.tex <==
\definecolor{Gray}{gray}{0.85}
\newcolumntype{a}{>{\columncolor{Gray}}c}
\begin{table*}[ht!]
\centering
\small
\begin{tabular}{llccccc|cc}
\toprule
         &         &               EM &               F1 &           Recall &           METEOR &          Rouge-L &       BertS (F1) &              BEM \\
Dataset & Model &                  &                  &                  &                  &                  &                  &                  \\
\midrule
\multirow{5}{*}{NQ} & FiD &     \textbf{46.57} &     \textbf{53.93} &            54.45 &     \textbf{42.94} &     \textbf{54.33} &     \textbf{92.57} &            58.81 \\
         & GPT-3.5 &             1.41 &            16.22 &  \underline{57.98} &            26.67 &            15.63 &            83.37 &     \textbf{70.01} \\
         & Flan-T5 &  \underline{41.16} &  \underline{50.62} &            54.03 &  \underline{40.80} &  \underline{51.02} &  \underline{91.77} &            58.74 \\
         & Alpaca &             8.84 &             19.5 &            48.82 &            21.62 &            19.82 &            84.23 &            57.22 \\
         & Llama-2 &             0.64 &             9.78 &     \textbf{59.28} &             17.5 &             9.34 &            81.63 &  \underline{64.66} \\
\midrule
\multirow{5}{*}{HotpotQA} & FiD &  \underline{48.43} &  \underline{60.16} &            60.55 &  \underline{46.03} &  \underline{60.18} &  \underline{93.02} &            67.94 \\
         & GPT-3.5 &             5.66 &            22.49 &            66.77 &            31.95 &            21.96 &            84.24 &  \underline{78.36} \\
         & Flan-T5 &     \textbf{58.12} &     \textbf{71.14} &     \textbf{71.28} &     \textbf{53.44} &     \textbf{71.16} &     \textbf{94.37} &            76.19 \\
         & Alpaca &            16.27 &            33.45 &            57.53 &            33.11 &            33.41 &            86.88 &            68.21 \\
         & Llama-2 &             1.39 &            15.15 &  \underline{69.75} &            26.45 &            14.51 &             82.9 &     \textbf{79.43} \\
\midrule
\multirow{5}{*}{TopiOCQA} & FiD &     \textbf{36.48} &     \textbf{58.52} &  \underline{61.64} &     \textbf{52.46} &     \textbf{58.26} &     \textbf{92.37} &  \underline{66.56} \\
         & GPT-3.5 &              2.7 &            34.32 &     \textbf{67.39} &  \underline{45.74} &            31.99 &            88.03 &     \textbf{69.26} \\
         & Flan-T5 &  \underline{18.34} &  \underline{43.17} &            52.54 &            42.42 &  \underline{42.88} &  \underline{89.42} &            56.57 \\
         & Alpaca &             5.85 &            26.72 &            43.37 &             29.9 &            25.85 &            86.73 &            47.03 \\
         & Llama-2 &             0.95 &            22.79 &             61.4 &            33.91 &            21.04 &            84.87 &            58.21 \\
\bottomrule
\end{tabular}


\caption{Performance of retrieval-augmented instruction-following models on three diverse information-seeking QA tasks. Among the metrics reported, \textit{Recall} is most correlated with human judgements. Based on recall, instruciton-following models outperform fine-tuned FiD on all three tasks.}

\label{tab:correctness_main_results}
\end{table*}

==> Tables/faithfulness_human_eval_metrics.tex <==
\setlength{\tabcolsep}{4.0pt}
\begin{table}[t!]
\centering
\small
\begin{tabular}{lccc}
\toprule
{} &   K-F1 &  K-Precision &  \multirowcell{2}{LLMCritic\\ (GPT-4)}\\
            &        &              &                    \\
\midrule
Faithful=1.0 $\uparrow$    &  0.20 &         0.88 &               0.98 \\
Not Faithful=0.0 $\downarrow$  &  0.23 &         0.51 &               0.57 \\
\bottomrule
\end{tabular}

\caption{Average scores from various evaluation metrics aggregated over samples evaluated by annotators. K-F1 assigns low scores to both faithful and unfaithful model responses. K-Precision and LLMCritic align better with human judgments.}
\label{tab:faithfulness_human_eval_metrics}
\end{table}

==> Tables/faithfulness_results.tex <==

\begin{table*}[ht]
\centering
\small
\begin{tabular}{llcc|cccc}
\toprule
         &         &             K-F1 $\uparrow$ &      K-Precision $\uparrow$ &     K-BertS (F1) $\uparrow$ &          $Q^2$ (F1) $\uparrow$ &         $Q^2$ (NLI) $\uparrow$ &      FaithCritic $\downarrow$ \\
Dataset & Model &                  &                  &                  &                  &                  &                  \\
\midrule
\multirow{4}{*}{NQ} & GPT-3.5 &  \underline{18.64} &            65.46 &  \underline{85.25} &  \underline{37.01} &  \underline{41.86} &     \textbf{19.44} \\
         & Flan-T5 &             5.84 &     \textbf{94.04} &             80.9 &            36.54 &            38.27 &            82.42 \\
         & Alpaca-7B &            15.98 &            69.36 &            83.72 &            30.94 &            33.91 &            68.75 \\
         & Llama-2 &     \textbf{23.90} &  \underline{69.37} &     \textbf{85.40} &     \textbf{38.93} &     \textbf{43.97} &  \underline{30.09} \\
\midrule
\multirow{4}{*}{HotpotQA} & GPT-3.5 &  \underline{16.17} &            81.41 &     \textbf{84.14} &  \underline{48.62} &  \underline{55.35} &  \underline{39.07} \\
         & Flan-T5 &             3.26 &     \textbf{92.12} &            78.57 &            36.03 &            37.97 &            64.31 \\
         & Alpaca-7B &            10.42 &  \underline{87.05} &            82.82 &            43.74 &            49.19 &            49.68 \\
         & Llama-2 &     \textbf{20.67} &             75.8 &  \underline{84.08} &     \textbf{49.19} &     \textbf{55.72} &     \textbf{37.58} \\
\midrule
\multirow{4}{*}{TopiOCQA} & GPT-3.5 &  \underline{27.89} &  \underline{69.55} &  \underline{87.15} &  \underline{52.92} &  \underline{58.50} &     \textbf{28.38} \\
         & Flan-T5 &            23.74 &     \textbf{86.37} &            86.42 &     \textbf{61.30} &     \textbf{64.75} &            44.89 \\
         & Alpaca-7B &            27.49 &            66.76 &            86.22 &            42.46 &            46.17 &            54.41 \\
         & Llama-2 &     \textbf{35.13} &            65.38 &     \textbf{87.88} &            49.48 &             53.8 &  \underline{36.30} \\
\bottomrule
\end{tabular}

\caption{Results for faithfulness w.r.t relevant knowledge. We report both token-based and model-based metrics. For all metrics except FaithCritic, higher scores indicate greater response groundedness.}
\label{tab:faithfulness_table}
\end{table*}

==> Tables/main_results.tex <==

\begin{table*}[ht!]
\centering
\small
\begin{tabular}{ll|ccc|cc|cc}
\toprule
         &         &               EM $\uparrow$ &               F1 $\uparrow$ &           Recall $\uparrow$ &             K-F1 $\uparrow$ &      K-Precision $\uparrow$ &   Incorrect Psg. $\uparrow$ &        Gold Psg. $\downarrow$ \\
Dataset & Model &                  &                  &                  &                  &                  &                  &                  \\
\midrule
\multirow{5}{*}{NQ} & FiD &     \textbf{46.57} &     \textbf{53.93} &            54.45 &               -- &               -- &               -- &               -- \\
         & Flan-T5 &  \underline{41.16} &  \underline{50.62} &            54.03 &             5.84 &     \textbf{94.04} &            91.99 &  \underline{24.76} \\
         & Alpaca &             8.84 &             19.5 &            48.82 &            15.98 &            69.36 &             0.03 &      \textbf{0.00} \\
         & GPT-3.5 &             1.41 &            16.22 &  \underline{57.98} &  \underline{18.64} &            65.46 &     \textbf{98.39} &            47.37 \\
         & Llama-2 &             0.64 &             9.78 &     \textbf{59.28} &     \textbf{23.90} &  \underline{69.37} &  \underline{97.76} &            57.76 \\
\midrule
\multirow{5}{*}{HotpotQA} & FiD &  \underline{48.43} &  \underline{60.16} &            60.55 &               -- &               -- &               -- &               -- \\
         & Flan-T5 &     \textbf{58.12} &     \textbf{71.14} &     \textbf{71.28} &             3.26 &     \textbf{92.12} &            77.14 &   \underline{1.58} \\
         & Alpaca &            16.27 &            33.45 &            57.53 &            10.42 &  \underline{87.05} &             0.08 &      \textbf{0.08} \\
         & GPT-3.5 &             5.66 &            22.49 &            66.77 &  \underline{16.17} &            81.41 &     \textbf{98.22} &            25.54 \\
         & Llama-2 &             1.39 &            15.15 &  \underline{69.75} &     \textbf{20.67} &             75.8 &  \underline{97.73} &            61.51 \\
\midrule
\multirow{5}{*}{TopiOCQA} & FiD &     \textbf{36.48} &     \textbf{58.52} &  \underline{61.64} &               -- &               -- &               -- &               -- \\
         & Flan-T5 &  \underline{18.34} &  \underline{43.17} &            52.54 &            23.74 &     \textbf{86.37} &            40.77 &   \underline{7.68} \\
         & Alpaca &             5.85 &            26.72 &            43.37 &            27.49 &            66.76 &             1.31 &      \textbf{0.84} \\
         & GPT-3.5 &              2.7 &            34.32 &     \textbf{67.39} &  \underline{27.89} &  \underline{69.55} &     \textbf{88.19} &            31.82 \\
         & Llama-2 &             0.95 &            22.79 &             61.4 &     \textbf{35.13} &            65.38 &  \underline{79.08} &            52.43 \\
\bottomrule
\end{tabular}

\caption{Main Results}

\label{tab:main_results}
\end{table*}

==> Tables/main_results_faithfulness_OLD.tex <==

\begin{table}[t!]
\centering
\footnotesize
\begin{tabular}{ll|c|cc}
\toprule
         &         &      \multirowcell{2}{K-Pre-\\cision $\uparrow$} &   \multirowcell{2}{Incorrect \\Psg. $\uparrow$} &        \multirowcell{2}{Gold \\Psg. $\downarrow$} \\
Dataset & Model &                  &                  &                  \\
\midrule
\parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{NQ}}} & Flan-T5 &     \textbf{94.04} &            91.99 &  \underline{24.76} \\
         & Alpaca &            69.36 &             0.03 &      \textbf{0.00} \\
         & GPT-3.5 &            65.46 &     \textbf{98.39} &            47.37 \\
         & Llama-2 &  \underline{69.37} &  \underline{97.76} &            57.76 \\
\midrule
\parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{HotpotQA}}} & Flan-T5 &     \textbf{92.12} &            77.14 &   \underline{1.58} \\
         & Alpaca &  \underline{87.05} &             0.08 &      \textbf{0.08} \\
         & GPT-3.5 &            81.41 &     \textbf{98.22} &            25.54 \\
         & Llama-2 &             75.8 &  \underline{97.73} &            61.51 \\
\midrule
\parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{TopiOCQA}}} & Flan-T5 &     \textbf{86.37} &            40.77 &   \underline{7.68} \\
         & Alpaca &            66.76 &             1.31 &      \textbf{0.84} \\
         & GPT-3.5 &  \underline{69.55} &     \textbf{88.19} &            31.82 \\
         & Llama-2 &            65.38 &  \underline{79.08} &            52.43 \\
\bottomrule
\end{tabular}

\caption{Main Results}

\label{tab:main_results_faithfulness}
\end{table}

==> Tables/prompt_sensitivity.tex <==
\begin{table}[t!]
\centering
\small
\begin{tabular}{llcc}
\toprule
         &         &         Instr. 1 &         Instr. 2 \\
Dataset & Model &                  &                  \\
\midrule
\multirow{4}{*}{NQ} & Flan-T5 &            54.03 &     \textbf{50.52} \\
         & Alpaca &            48.82 &  \underline{48.00} \\
         & GPT-3.5 &  \underline{57.98} &             34.1 \\
         & Llama-2 &     \textbf{59.28} &            44.03 \\
\midrule
\multirow{4}{*}{HotpotQA} & Flan-T5 &     \textbf{71.28} &     \textbf{69.68} \\
         & Alpaca &            57.53 &  \underline{57.37} \\
         & GPT-3.5 &            66.77 &            40.08 \\
         & Llama-2 &  \underline{69.75} &            47.56 \\
\midrule
\multirow{4}{*}{TopiOCQA} & Flan-T5 &            52.54 &     \textbf{49.16} \\
         & Alpaca &            43.37 &            42.85 \\
         & GPT-3.5 &     \textbf{67.39} &  \underline{46.76} \\
         & Llama-2 &  \underline{61.40} &            42.62 \\
\bottomrule
\end{tabular}


\caption{Prompt sensitivity table}
\label{tab:prompt_sensitivity}
\end{table}

==> Tables/unanswerability.tex <==
\begin{table}[t!]
\centering
\scriptsize
\begin{tabular}{llcc}
\toprule
         &         & Incorrect Psg. $\uparrow$ &    Gold Psg. $\downarrow$ \\
Dataset & Model &                &              \\
\midrule
\multirow{4}{*}{NQ} & GPT-3.5 &           98.5 &        48.01 \\
         & Flan-T5 &          91.99 &        24.76 \\
         & Alpaca &           0.06 &  \textbf{0.00} \\
         & Llama-2 &   \textbf{99.34} &        75.84 \\
\midrule
\multirow{4}{*}{HotpotQA} & GPT-3.5 &          98.54 &        26.39 \\
         & Flan-T5 &          77.14 &         1.58 \\
         & Alpaca &           0.09 &  \textbf{0.11} \\
         & Llama-2 &   \textbf{99.16} &        76.96 \\
\midrule
\multirow{4}{*}{TopiOCQA} & GPT-3.5 &   \textbf{88.15} &        32.42 \\
         & Flan-T5 &          40.77 &         7.68 \\
         & Alpaca &           1.27 &  \textbf{0.80} \\
         & Llama-2 &          87.59 &        61.77 \\
\bottomrule
\end{tabular}

\caption{Percentage of model responses that contain \emph{I don't know} and other synonymous expressions when provided with an incorrect passage (higher is better) or the gold passage (lower is better).}
\label{tab:unanswerability}
\end{table}
